Neptune: The Long Orbit to Benchmarking Long Video Understanding

We introduce Neptune, a benchmark for long video understanding that requires reasoning over long time horizons and across different modalities. Many existing video datasets and models are focused on short clips (10s-30s). While some long video datasets do exist, they can often be solved by powerful image models applied per frame (and often to very few frames) in a video, and are usually manually annotated at high cost. In order to mitigate both these problems, we propose a scalable dataset creation pipeline which leverages large models (VLMs and LLMs), to automatically generate dense, time-aligned video captions, as well as tough question answer decoy sets for video segments (up to 15 minutes in length). Our dataset Neptune covers a broad range of long video reasoning abilities and consists of a subset that emphasizes multimodal reasoning. Since existing metrics for open-ended question answering are either rule-based or may rely on proprietary models, we provide a new open source model-based metric GEM to score open-ended responses on Neptune. Benchmark evaluations reveal that most current open-source long video models perform poorly on Neptune, particularly on questions testing temporal ordering, counting and state changes. Through Neptune, we aim to spur the development of more advanced models capable of understanding long videos. The dataset is available at https://github.com/google-deepmind/neptune

==> datasheet.tex <==
Datasheets for datasets introduced by \citet{gebru2021datasheets} serve as a medium of communication between the creators and users of a dataset.
They effectively consolidate the motivation, creation process, composition, and intended uses of a dataset as a series of questions and answers.
In this Section, we provide a datasheet for the \dataset{} dataset.

\section*{Motivation}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{0}

\dsquestionex{For what purpose was the dataset created?}{Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.}
\label{Q1}

\dsanswer{
The \dataset{} dataset was created to test long video understanding via the medium of video question answering. This fills a gap in the current set of benchmarks available for video understanding, as most datasets are still focused on short-form video clips. We believe \dataset{} proposes a significant challenge for, and hence can provide key insights for the development of VLMs applied to long video understanding.
}

\dsquestion{Who created this dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}
\label{Q2}

\dsanswer{
The \dataset{} dataset was created by researchers at Google LLC.
}

\dsquestionex{Who funded the creation of the dataset?}{If there is an associated grant, please provide the name of the grantor and the grant name and number.}
\label{Q3}

\dsanswer{
The \dataset{} dataset was funded by Google LLC.
}

\dsquestion{Any other comments?}
\label{Q4}

\dsanswer{No.}

\end{compactenum}


\section*{Composition}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{4}
    
\dsquestionex{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}{ Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.}
\label{Q5}

\dsanswer{
Each instance in \dataset{} represents a YouTube video, and annotations in the form of question, answer and 4 decoys (QAD).
}

\dsquestion{How many instances are there in total (of each type, if appropriate)?}
\label{Q6}

\dsanswer{
There are \dsetsize{} instances in \dataset{}.
}

\dsquestionex{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}{ If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).}
\label{Q7}

\dsanswer{
\dataset{} is a small sample drawn from all the data uploaded to YouTube. 
Millions of videos are uploaded on YouTube every day.
We start from a subset of YouTube video candidates from the YT-Temporal-1Bn dataset~\cite{zellersluhessel2021merlot}, which is biased towards videos where the ASR has a strong correlation with the visual content. 
Our final subset (\dsetvideos{} videos) was created after a number of filtering and processing stages, which aim to increase the diversity of samples in the data.
Hence the \dataset{} data does not fully represent the distribution of videos uploaded to YouTube.
}

\dsquestionex{What data does each instance consist of? “Raw” data (e.g., unprocessed text or images) or features?}{In either case, please provide a description.}
\label{Q8}

\dsanswer{
Each instance in \dataset{} consists of four metadata fields:
\begin{compactitem}
\item \texttt{"video\_id"}: Unique alphanumeric ID of the video (assigned by YouTube).
\item \texttt{"url"}: Static URL for downloading the video, e.g., \texttt{https://www.youtube.com/watch?v=<video\_id>}.
\item \texttt{"question"}: A hard question about the video.
\item \texttt{"answer"}: An answer to the above question.
\item \texttt{"decoys"}: Four decoy answers intended to be used in conjunction with the question and answer for multiple choice evaluation.
\end{compactitem}
}

\dsquestionex{Is there a label or target associated with each instance?}{If so, please provide a description.}
\label{Q9}

\dsanswer{
We provide QADs, though it might also be also possible to use auxiliary
information (like video titles or tags).
}

\dsquestionex{Is any information missing from individual instances?}{If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g., redacted text.}
\label{Q10}

\dsanswer{
No and yes.
No, because all the metadata fields for every instance are filled with valid values.
Yes, because the \texttt{"url"} for some instances may not retrieve the underlying video.
This may happen if the YouTube user (author) removes the video from YouTube.
Such deletions reduce our dataset size over time, however, video deletions are rare.
}

\dsquestionex{Are relationships between individual instances made explicit (e.g., users’ movie ratings, social network links)?}{If so, please describe how these relationships are made explicit.}
\label{Q11}

\dsanswer{
Relationships between individual instances (e.g., videos made by the same creator) are not made explicit in our work, though this is a possibility for future work.
}

\dsquestionex{Are there recommended data splits (e.g., training, development/validation, testing)?}{If so, please provide a description of these splits, explaining the rationale behind them.}
\label{Q12}

\dsanswer{
Our entire dataset is meant to be a test set only. We provide challenging subsets (MMA and MMH) focusing on videos that require multimodal understanding by LLMs and humans, respectively.
}

\dsquestionex{Are there any errors, sources of noise, or redundancies in the dataset?}{If so, please provide a description.}
\label{Q13}

\dsanswer{
\dataset{} may be noisy as each QAD annotation was created automatically by machine learning methods first. While each annotation has been checked by a human rater, there may be some unavoidable human error in the annotation process. 
}

\dsquestionex{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?}{If it links to or relies on external resources,
\begin{compactenum}[\hspace{1pt}(a)]
    \item Are there guarantees that they will exist, and remain constant, over time?
    \item Are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created)?
    \item Are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a future user? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.
\end{compactenum}}
\label{Q14}

\dsanswer{
The dataset relies on videos hosted on YouTube. We do not distribute videos of our dataset to respect YouTube's terms of service. 
Instead, we provide video URLs (\texttt{"url"}, \qref{Q8}) that point to videos hosted on YouTube servers.
In response to sub-questions:
\begin{compactenum}[\hspace{1pt}(a)]
    \item There are no guarantees that videos will remain available on YouTube.
    \item There are no archived versions of the dataset.
    \item We refer to the YouTube ToS for details on content restrictions \href{https://www.youtube.com/static?template=terms}{https://www.youtube.com/static?template=terms}.
\end{compactenum}
}

\dsquestionex{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals non-public communications)?}{If so, please provide a description.}
\label{Q15}

\dsanswer{
No, the videos included in \dataset{} do not cover topics that may be considered confidential.
All videos were publicly shared on YouTube prior to inclusion in \dataset{}.
}

\dsquestionex{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}{If so, please describe why.}
\label{Q16}

\dsanswer{
While we cannot be certain that our raters were able to remove all videos mentioned above, we explicitly ask them to do so in their annotation guidelines. We also note that YouTube removes videos that contain offensive content or do not follow their community guidelines.
}

\dsquestionex{Does the dataset relate to people?}{If not, you may skip remaining questions in this section.}
\label{Q17}

\dsanswer{
The dataset pertains to people in that people have uploaded the videos to YouTube.
Furthermore, most videos in \dataset{} have people speaking and/or appearing.
}

\dsquestionex{Does the dataset identify any subpopulations (e.g., by age, gender)?}{If so, please describe how these subpopulations are identified and provide a description of their respective distributions within the dataset.}
\label{Q18}

\dsanswer{
\dataset{} does not explicitly identify any subpopulations.
Since most videos contain people and questions are free-form natural language questions produced by automatic machine learning models, it is possible that some annotations may identify people appearing in individual videos as part of a subpopulation.
}

\dsquestionex{Is it possible to identify one or more natural persons, either directly or indirectly (i.e., in combination with other data) from the dataset?}{If so, please describe how.}
\label{Q19}

\dsanswer{
Yes, our data includes celebrities, or other YouTube-famous people. 
All of the videos that we use are of publicly available data, following the Terms of Service (\url{https://www.youtube.com/static?template=terms}) that users agreed to when uploading to YouTube.
}

\dsquestionex{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?}{If so, please provide a description.}
\label{Q20}

\dsanswer{
This is highly unlikely, as YouTube removes videos that contain offensive content or do not follow their community guidelines.
}

\dsquestion{Any other comments?}
\label{Q21}

\dsanswer{No.}

\end{compactenum}


\section*{Collection Process}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{21}

\dsquestionex{How was the data associated with each instance acquired?}{Was the data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.}
\label{Q22}

\dsanswer{
See \qref{Q7} for an explanation of how the candidate video IDs were chosen.
These video IDs were provided by the YT-Temporal-1Bn dataset providers~\cite{zellersluhessel2021merlot} and then filtered by our automatic filtering process decribed in the main paper. 
The \texttt{"video\_id"} and \texttt{"URL"} are directly observable from YouTube. 
The annotations were obtained by machine learning models and then verified by human annotators. 
}

\dsquestionex{What mechanisms or procedures were used to collect the data (e.g., hardware apparatus or sensor, manual human curation, software program, software API)?}{How were these mechanisms or procedures validated?}
\label{Q23}

\dsanswer{
We collected all data using compute resources provided by Google LLC. The code involved running various machine learning models to obtain the annotations.
The code was validated by checking several data samples from \dataset{}. All annotations were then verified by human raters.
}

\dsquestion{If the dataset is a sample from a larger set, what was the sampling strategy?}
\label{Q24}

\dsanswer{
See \qref{Q7}.
}

\dsquestion{Who was involved in data collection process (e.g., students, crowd-workers, contractors) and how were they compensated (e.g., how much were crowd-workers paid)?}
\label{Q25}

\dsanswer{
The first few stages of our data collection pipeline are fully automatic and do not require any human annotators. The final stage involved contractor raters. 
}

\dsquestionex{Over what timeframe was the data collected? Does this timeframe match the creation timeframe of the data associated with the instances (e.g., recent crawl of old news articles)?}{If not, please provide a description of the timeframe.}
\label{Q26}

\dsanswer{
We collected all data in early 2024. As mentioned in Q22, videos are sampled from the YT-Temporal-1Bn dataset~\cite{zellersluhessel2021merlot} which was collected in 2021 so videos are uploaded no later than 2021.
}

\dsquestionex{Were any ethical review processes conducted (e.g., by an institutional review board)?}{If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.}
\label{Q27}

\dsanswer{
We did not conduct a formal ethical review process via institutional review boards.
However, as described in \if\sepappendix1{\textcolor{red}{Section 3.3} of the main paper }\else{\textcolor{red}{Section~\ref{sec:video-selection-signal-extraction} }}\fi and \qref{Q16} we employed several filtering mechanisms to tag instances that could be problematic.
}

\dsquestionex{Does the dataset relate to people?}{If not, you may skip remaining questions in this section.}
\label{Q28}

\dsanswer{
Yes, see \qref{Q17}.
}

\dsquestion{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g., websites)?}
\label{Q29}

\dsanswer{
We collected data submitted by YouTube users indirectly through the YouTube API.
However, users agree with YouTube's Terms of Service regarding the redistribution of their data by YouTube.
}

\dsquestionex{Were the individuals in question notified about the data collection?}{If so, please describe (or show with screenshots or other information) how notice was provided, and provide a link or other access point to, or otherwise reproduce, the exact language of the notification itself.}
\label{Q30}

\dsanswer{
Users were not notified about to the use of their data in our dataset.
However, by uploading their data on YouTube, they consent that it would appear on the YouTube platform and will be accessible via the official YouTube API (which we use to collect \dataset{}).
}

\dsquestionex{Did the individuals in question consent to the collection and use of their data?}{If so, please describe (or show with screenshots or other information) how consent was requested and provided, and provide a link or other access point to, or otherwise reproduce, the exact language to which the individuals consented.}
\label{Q31}

\dsanswer{
See \qref{Q30}.
}

\dsquestionex{If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?}{If so, please provide a description, as well as a link or other access point to the mechanism (if appropriate).}
\label{Q32}

\dsanswer{
Users have full control over the presence of their data in our dataset.
If users delete the underlying YouTube video -- it will be automatically removed from \dataset{} since we distributed videos as URLs.
}

\dsquestionex{Has an analysis of the potential impact of the dataset and its use on data subjects (e.g., a data protection impact analysis) been conducted?}{If so, please provide a description of this analysis, including the outcomes, as well as a link or other access point to any supporting documentation.}
\label{Q33}

\dsanswer{No.}

\dsquestion{Any other comments?}
\label{Q34}

\dsanswer{No.}

\end{compactenum}


\section*{Preprocessing, Cleaning, and/or Labeling}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{34}

\dsquestionex{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?}{If so, please provide a description. If not, you may skip the remainder of the questions in this section.}
\label{Q35}

\dsanswer{
After human raters annotated the dataset, we ran the following postprocessing and cleaning stages - blind and ASR cleaning. Details are provided in the main paper.
}

\dsquestionex{Was the ``raw'' data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?}{If so, please provide a link or other access point to the “raw” data.}
\label{Q36}

\dsanswer{
No, we only provide the filtered data.
}

\dsquestionex{Is the software used to preprocess/clean/label the instances available?}{If so, please provide a link or other access point.}
\label{Q37}

\dsanswer{
The exact model used is not available, but we explain the process in detail in the paper, allowing other researchers to reproduce our pipeline. 
}

\dsquestion{Any other comments?}
\label{Q38}

\dsanswer{No.}

\end{compactenum}


\section*{Uses}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{38}

\dsquestionex{Has the dataset been used for any tasks already?}{If so, please provide a description.}
\label{Q39}

\dsanswer{
We have only used the dataset to evaluate machine learning models as described in the paper. 
}

\dsquestionex{Is there a repository that links to any or all papers or systems that use the dataset?}{If so, please provide a link or other access point.}
\label{Q40}

\dsanswer{
We do not maintain such a repository.
However, citation trackers like Google Scholar and Semantic Scholar would list all future works that cite our dataset.
}

\dsquestion{What (other) tasks could the dataset be used for?}
\label{Q41}

\dsanswer{The dataset can only be used to evaluate video question answering.}

\dsquestionex{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?}{For example, is there anything that a future user might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other undesirable harms (e.g., financial harms, legal risks) If so, please provide a description. Is there anything a future user could do to mitigate these undesirable harms?}
\label{Q42}

\dsanswer{
This is very difficult to anticipate.
Future users of our dataset should be aware of YouTube's user demographics 
which might subtly influence the types of videos, languages, and ideas that are present in the dataset.
Also, note that our dataset is mainly composed of English videos, hence models trained on this dataset might perform worse on videos in other languages.
}

\dsquestionex{Are there any tasks for which the dataset should not be used?}{If so, please provide a description.}
\label{Q43}

\dsanswer{
Broadly speaking, our dataset should only be used for evaluating models. 
Our dataset should not be used for any tasks that involve identifying features related to people (facial recognition, gender, age, ethnicity identification, etc.) or making decisions that impact people (mortgages, job applications, criminal sentences; or moderation decisions about user-uploaded data that could result in bans from a website).
}

\dsquestion{Any other comments?}
\label{Q44}

\dsanswer{No.}

\end{compactenum}


\section*{Distribution}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{44}

\dsquestionex{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}{If so, please provide a description.}
\label{Q45}

\dsanswer{
Yes, our dataset is publicly available.
}

\dsquestionex{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)}{Does the dataset have a digital object identifier (DOI)?}
\label{Q46}

\dsanswer{
We distribute our dataset as a JSON file containing annotations hosted on GitHub.
Users will have to download the videos by themselves. All uses of \dataset{} should cite the paper as the reference.
}

\dsquestion{When will the dataset be distributed?}
\label{Q47}

\dsanswer{
The dataset is publicly available at \href{https://github.com/google-deepmind/neptune}{https://github.com/google-deepmind/neptune}.
}

\dsquestionex{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}{If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.}
\label{Q48}

\dsanswer{
Uses of our dataset are subject to YouTube API terms (\url{https://www.youtube.com/static?template=terms}).
This data is licensed by Google Inc. under a Creative Commons Attribution 4.0 International License. Users are allowed to modify and repost it, and we encourage them to analyze and publish research based on the data.
}

\dsquestionex{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}{If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.}
\label{Q49}

\dsanswer{
The videos corresponding to our instances are legally owned by YouTube users. Use of the dataset and containing videos are subject to YouTube ToS (\url{https://www.youtube.com/static?template=terms}).
}

\dsquestionex{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}{If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.}
\label{Q50}

\dsanswer{No.}

\dsquestion{Any other comments?}
\label{Q51}

\dsanswer{No.}

\end{compactenum}


\section*{Maintenance}

\begin{compactenum}[\hspace{0pt}Q1.]
\setcounter{enumi}{51}

\dsquestion{Who will be supporting/hosting/maintaining the dataset?}
\label{Q52}

\dsanswer{
The authors will maintain the dataset.
The dataset is hosted on Google cloud.
All the information about the dataset, including links to the paper and future announcements will be accessible at the dataset website on GitHub.
}

\dsquestion{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}
\label{Q53}

\dsanswer{The contact emails of authors are available on the dataset website.}

\dsquestionex{Is there an erratum?}{If so, please provide a link or other access point.}
\label{Q54}

\dsanswer{
There is no erratum for our initial release.
We will version all errata as future releases (\qref{Q55}) and document them on the dataset website.
}

\dsquestionex{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}{If so, please describe how often, by whom, and how updates will be communicated to users (e.g., mailing list, GitHub)?}
\label{Q55}

\dsanswer{
We will update our dataset periodically and announce updates on the dataset website.
These future versions would remove instances that were requested to be removed via the opt-out form (\qref{Q32}).
}

\dsquestionex{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were individuals in question told that their data would be retained for a fixed period of time and then deleted)?}{If so, please describe these limits and explain how they will be enforced.}
\label{Q56}

\dsanswer{
Rather than directly distributing videos, we distribute URLs that point to the original videos uploaded by YouTube users.
This means that users retain full control of their data -- any post deleted from YouTube will be automatically removed from \dataset{} (see also \qref{Q10}, \qref{Q14}, \qref{Q31}).
}

\dsquestionex{Will older versions of the dataset continue to be supported/hosted/maintained?}{If so, please describe how. If not, please describe how its obsolescence will be communicated to users.}
\label{Q57}

\dsanswer{
A new version release of \dataset{} will automatically deprecate its previous version.
We will only support and maintain the latest version at all times.
We decided to deprecate old versions to ensure that any data that is requested to be removed (\qref{Q32}) will be no longer accessible in future versions.
}

\dsquestionex{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}{If so, please provide a description. Will these contributions be verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to other users? If so, please provide a description.}
\label{Q58}

\dsanswer{
Anyone can extend \dataset{} by using our automatic pipeline described in the main paper.
}
\end{compactenum}

